Anchor Free IP Mobility

Efficient mobility management techniques are critical in providing seamless connectivity and session continuity between a mobile node and the network during its movement. Current mobility management solutions generally require a central entity in the network core, tracking IP address movement and anchoring traffic from source to destination through point-to-point tunnels. Intuitively, this approach suffers from scalability limitations as it creates bottlenecks in the network, due to sub-optimal routing via the anchor point. Meanwhile, alternative anchorless, solutions are not feasible due to the current limitations of the IP semantics, which strongly ties addressing information to location. In contrast, novel path-based forwarding solutions may be exploited for feasible anchorless solutions. In this paper, we propose a novel network-based mobility management solution that facilitates IP mobility over such a path-based forwarding substrate. Our solution exploits the advantages of such substrates in decoupling path calculation from data transfer to eliminate the need for anchoring traffic through the network core; thereby, allowing flexible path calculation and service provisioning. Furthermore, by eliminating the limitation of routing via the anchor point, our approach reduces the network cost compared to anchored solution through bandwidth saving while maintaining comparable handover delay. We evaluate our solution through analytical and simulation models and compare it with the IETF standardized solution, Proxy Mobile IPv6 (PMIPv6). Evaluation results illustrate a significant saving in the total network cost when using our proposed solution, compared to its counterpart.

==> README <==

September 17, 2014


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society journal subset of the full
IEEEtran package and is intended for use with Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8a has a number of significant changes over the v1.8 release.
For a full list of changes, please read the file changelog.txt. The most
notable changes include:


 1) Extensive rework of the compsoc mode to comply with the latest standards
    of the IEEE Computer Society.

 2) Fixed abstract, index terms and diamond line for compsoc technotes.

 3) New \IEEEraisesectionheading{} command to provide for the special
    raised first section heading of Computer Society journal papers.

 4) Internal code improvements for page setup and command argument
    processing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_jrnl_compsoc.tex.
***************************************************************************

